Next-to-leading order QCD and electroweak corrections to Higgs-strahlung processes at the LHC

In this paper we calculate the total and fiducial cross sections as well as differential distributions for the Higgs-strahlung or VH process $p p \to VH \to l\nu_l/l^- l^+ + H$, (V = W or Z, l=e,$\mu$) including QCD and electro-weak corrections up to next-to-leading order before and after reweighting photon PDFs of NNPDF2.3qed, NNPDF3.0qed, MRST2004qed, CT14QEDinc, and LUXqed at the LHC with 13 TeV and Higgs boson mass $\ M_{H}=125$ GeV. The predictions from the various photon PDFs before and after reweighting against each other are in good agreement. The photon PDF uncertainties of the photon-induced cross sections decrease significantly with the reweighting PDFs.

==> feynmanDiagramTikz.tex <==

	\begin{tabular}{cc}
		\begin{tikzpicture}[
					thick,
			% Set the overall layout of the tree
			level/.style={level distance=2.0cm, line width=0.4mm},
			level 2/.style={sibling angle=60},
			level 3/.style={sibling angle=60},
			level 4/.style={level distance=2cm, sibling angle=60}
	]
			\coordinate
			child[grow=-30]{
				child[grow=east] { 
					child[grow=-30] {    		
						edge from parent [electron]
						node[below=3pt] {$d$}    
					}
					child[grow=30] {
						edge from parent [electron2]
						node [above] {$\bar{d}$}
					}
					child[grow=90] {
						edge from parent [gluon]
						node [above] {$g$}
					}    
		  			edge from parent [gluon]
		   			node[above=3pt] {$g$}           
		 		}
				child[grow=210] {
		   			edge from parent [electron]
		   			node[below=3pt] {$\bar{u}$}
		 		}
		 		edge from parent [electron] node [above=3pt] {$u$}
			};
		\end{tikzpicture}   
				\hspace{12 mm}
		&
		\begin{tikzpicture}[
					thick,
			% Set the overall layout of the tree
			level/.style={level distance=2.0cm, line width=0.4mm},
			level 2/.style={sibling angle=60},
			level 3/.style={sibling angle=60},
			level 4/.style={level distance=2cm, sibling angle=60}
	]
			\coordinate
			child[grow=-30]{
				child[grow=east] { 
					child[grow=-30] {    		
						edge from parent [electron]
						node[below=3pt] {$e^-$}    
					}
					child[grow=30] {
						edge from parent [electron2]
						node [above] {$e^+$}
					}    
		  			edge from parent [boson]
		   			node[above=3pt] {$Z/\gamma^*$}           
		 		}
				child[grow=210] {
		   			edge from parent [electron]
		   			node[below=3pt] {$\bar{u}$}
		 		}
		 		edge from parent [electron] node [above=3pt] {$u$}
			};
		\end{tikzpicture}
	 \end{tabular}



         
